Using Deep Reinforcement Learning for mmWave Real-Time Scheduling

We study the problem of real-time scheduling in a multi-hop millimeter-wave (mmWave) mesh. We develop a model-free deep reinforcement learning algorithm called Adaptive Activator RL (AARL), which determines the subset of mmWave links that should be activated during each time slot and the power level for each link. The most important property of AARL is its ability to make scheduling decisions within the strict time slot constraints of typical 5G mmWave networks. AARL can handle a variety of network topologies, network loads, and interference models, it can also adapt to different workloads. We demonstrate the operation of AARL on several topologies: a small topology with 10 links, a moderately-sized mesh with 48 links, and a large topology with 96 links. We show that for each topology, we compare the throughput obtained by AARL to that of a benchmark algorithm called RPMA (Residual Profit Maximizer Algorithm). The most important advantage of AARL compared to RPMA is that it is much faster and can make the necessary scheduling decisions very rapidly during every time slot, while RPMA cannot. In addition, the quality of the scheduling decisions made by AARL outperforms those made by RPMA.

==> files/3-RL.tex <==
Reinforcement Learning is a machine learning (ML) framework in which an agent repeatedly interacts with an environment and is trained to maximize a cumulative reward \cite{article111, inproceedings2222, 10.1145/3152434.3152441}. RL is one of the most important ML paradigms, alongside with supervised and unsupervised learning. A particularly successful embodiment of RL is deep RL, which makes use of deep neural network models. This section describes the basic RL notions and tools, which are used for addressing the routing problem.\\

RL is concerned with temporal processes where time is modeled to be discrete. Unlike its other machine learning cousins, RL does not require labeled input/output pairs or sub-optimal actions to be explicitly corrected; instead, it is concerned with finding a balance between acquiring new knowledge (exploration) and using current knowledge (exploitation) about the environment and the agent's optimal behavior. The environment is modeled as a Markov Decision Process, defined as a tuple $(S, A,\sigma,r,S_\mathrm{T})$. $S$ and $A$ denote the sets of environment states and actions that can be applied by the agent respectively; $\sigma$ : $S \times A\rightarrow S$ denotes the state transition function, which determines how actions affect the environment state; $r : SxA \rightarrow \mathbb{R}$ denotes the reward function, which assigns a scalar score (reward) to an action taken by the agent; and $S_\mathrm{T}$ denotes the terminal states that stop the process \cite{kaelbling1996reinforcement}.\\

%An episode is a sequence of $s_{0},a_{0},r_{0}, s_{1},a_{1},r_{1},\dots,s_{n}$ states, actions and rewards, starting from an initial state $s_{0}$ and ending at a terminal state $s_{n} \in S_\mathrm{T}$. In each step $i=0,\dots,n-1$, the agent receives the current state $s_{i} \in S$ and chooses an action $a_{i} \in A$. Then for taking $a_i$, the environment generates the reward $r_{i} = r(s_{i},a_{i})$ and the next state $s_{i+1}=\sigma(s_{i},a_{i})$, which are communicated to the agent as feedback. A policy is a function $\pi : S\rightarrow A$, which chooses an action $a \in A$ for any given state. A policy can also be stochastic, in which case $\pi$ is interpreted as a conditional distribution $\pi(a|s)$, and the action is sampled from it.\\
RL aims to maximize the expected cumulative reward by finding the agent's optimal policy. 
To find the optimal policy, it is  critical to determine the value of each state-action function, also known as the Q-function: $Q_\pi(s,a) = \E_\pi [ G_t| S_t=s,A_t = a]=R_s^{a}+\gamma\sum_{s' \in S}P_{ss'}^{a}v_\pi(s'),$
% \begin{equation}
% \begin{gathered}
% Q_\pi(s,a) = \E_\pi [ G_t| S_t=s,A_t = a]=R_s^{a}+\gamma\sum_{s' \in S}P_{ss'}^{a}v_\pi(s'),
% \nonumber
% \end{gathered}
% \end{equation}
%$Q_\pi(s,a) = \E_\pi [ G_t| S_t=s,A_t = a]=R_s^{a}+\gamma\sum_{s' \in S}P_{ss'}^{a}v_\pi(s'),$
where  $R_s^{a}$ is the instant reward that can be obtained by taking
action \(a\) under state \(s\); \(P_{ss'}^{a}\) is the transition probability from state \(s\) to state $s'$ under action \(a\); \(\gamma\) is the discount factor used to balance the long-term and short-term rewards; and \(G_t\) is the cumulative reward from time \(t\), given by $G_t= \sum_{k=0}^{\infty} \gamma^{k} R_{t+k+1}.$
$v_\pi(s) = \E_{\pi} [G_t| s_t=s] = \sum_{a \in A} \pi(a|s)Q_{\pi}(s|a)$. In the case of small state-action spaces, the Q-function can be simply computed and tabulated. However, such an approach quickly becomes infeasible as the cardinality of $S$ and $A$ grows. Deep neural networks were shown to be spectacularly successful in approximating the values of $Q$, with a reasonable number of trainable parameters.\\
There are two approaches to RL problems: model-based and model-free. Model-based learning models the environment and then chooses the optimal policy based on the learned model. In model-free learning, the agent establishes the optimal policy through trial and error, \cite{9634122}. Model-free methods are classified into two broad categories: policy optimization techniques and Q-learning value iteration techniques. In policy optimization, the agent directly learns the policy function that maps state to action, without the use of the value function. Among the algorithms that make use of this method is Trust Region Policy Optimization (TRPO) \cite{schulman2017trust}. It is an on-policy method, which means that it attempts to evaluate or improve the policy that is currently being used to take actions, and it uses information gathered from consecutive steps. It is applicable to both discrete and continuous action spaces, and it updates policies by taking the most significant possible step to improve performance while adhering to a unique constraint on the degree of similarity between the new and the old policies. The constraint ensures that the new updated policy is not too far removed from the old policy, implying that the new policy is within the trust region of the old policy:\\
\begin{equation}
\begin{gathered}
\begin{multlined}
    \max_{\pi'} \E_{\pi'} \left[ \frac{\pi'(a|s)}{\pi(a|s)} \hat{A}_{\pi}(s,a) \right], \\ \mathrm{s.t.} \,\,  \E_{\pi}[D_\mathrm{KL}(\pi(\cdot|s) \, | \, \pi' (\cdot|s))]\leq\delta,
\end{multlined}
\end{gathered}
\label{KL}
\end{equation}where $\pi'$ and $\pi$ denote the new and the previous policies. $\hat{A}_{\pi}(s,a) \approx Q_{\pi}(s,a) - v_\pi(s) $
%$\hat{A}_{\pi}(s,a) \approx Q_{\pi}(s,a) - v_\pi(s)$ 
% \begin{equation}
% \begin{gathered}
% \hat{A}_{\pi}(s,a) \approx Q_{\pi}(s,a) - v_\pi(s) 
% \nonumber
% \end{gathered}
% \end{equation} 
is the approximate advantage function (i.e., the gain in reward relative to the state value when taking a specific action $a$), $D_\mathrm{KL}$ is the Kullback-Leibler (KL) divergence between two distributions, and $\delta$ is a fixed radius. The policy and advantage functions are implemented in practical DRL implementations as neural networks parameterized by some parameter vector $\theta$. Eq. \ref{KL} can be interpreted as maximizing the objective function that meets the KL constraint term on the policy update step size. The KL constraint adds additional overhead in the form of hard restrictions to the optimization process. The probability ratio between the new policy $\pi_{\theta'}$ and the old one $\pi_{\theta}$ is defined as 
\begin{equation}
r({\theta}') = \frac{\pi_{\theta'}(a|s)}{\pi_{\theta}(a|s)}.
\nonumber
\end{equation}
TRPO's objective function is then defined as $J_{\textrm{TRPO}}(\theta') = \E \left[ r({\theta'}) A_{\theta'}(s,a)\right]$.
% \begin{equation}
% \begin{gathered}
% J_{\textrm{TRPO}}(\theta') = \E \left[ r({\theta'}) A_{\theta'}(s,a)\right].
% \nonumber
% \end{gathered}
% \end{equation}
% \begin{equation}
% \begin{gathered}
% J_{\textrm{TRPO}}(\theta') = \E \left[ r({\theta'}) A_{\theta'}(s,a)\right].
% \nonumber
% \end{gathered}
% \end{equation}
Like TRPO, Proximal Policy Optimization (PPO) \cite{schulman2017proximal}, is also an on-policy algorithm that can be applied to discrete or continuous actions spaces. It seeks to improve the policy without risking performance collapse. Moreover, by limiting policy updates at each training step, PPO improves the stability of the agent's training. It is a first-order optimization. In the absence of constraints, the large and small step size updates of the objective function, can cause instability or slow convergence. To stay within a small interval around $1$, PPO replaces the complex KL constraint from Eq. \ref{KL} with clipping the policy ratio $r$ \cite{schulman2017proximal},
\begin{equation}
\begin{multlined}
\begin{gathered}
J_\textrm{PPO}(\theta') = \E\left[ \min\{ r({\theta}'), 1+\epsilon\} \hat{A}_{\theta}(s,a)\right].
\nonumber
\end{gathered}
\end{multlined}
\end{equation}
The clipping at $1+\epsilon$ ensures that $J_\textrm{PPO}$ lower bounds $J_{\textrm{TRPO}}$.






==> files/future.tex <==
In the future, we intend to develop a more optimized architecture for each topology. As is often the case with other deep learning methods, developing such an architecture that is tailored to a specific use-case \cite{zhang2017zipnet,8666641}, in our case a topology, can help improve the DRL algorithm's performance. In our work, we used a simple neural network architecture with only two hidden layers and an equal number of neurons in each layer. We used a different size hidden layer for each topology. Developing a tailored architecture could significantly improve the agent's ability to learn how to schedule and set the power level. Adding additional layers of varying sizes could alter the training time and enhance the performance of real-time decisions.\\ 

Another approach that might be taken is to use Graph Neural Networks' (GNN) topology extraction capabilities \cite{scarselli2008graph}. GNN takes a graph with node and edge features as input and computes a function that is dependent on both the features and the graph structure. GNN has the capability to extract topological structures and properties. Message-passing GNNs (MPNN) propagate graph properties by sharing information between nearby nodes. Each node in a typical MPNN architecture is updated based on the aggregation of its neighbors' features. By using GNN, the DRL agent may be able to better learn the topology and hence increase its performance.

==> files/new-RL.tex <==
In this section, we provide a brief introduction to DRL. We consider a typical RL setup consisting of an agent interacting with an environment in discrete decision steps. At each decision step $t$, the agent observes the environment's state $s_t$, takes an action $a_t$ and, as a consequence receives a reward $r_t$ from the environment. The environment is modeled as a Markov Decision Process, defined as a tuple $(S, A,\sigma,r,S_\mathrm{T})$. $S$ and $A$ denote the sets of the environment states and the actions that can be applied by the agent, respectively; $\sigma$ : $S \times A\rightarrow S$ denotes the state transition function, which determines how actions affect the environment state; $r : SxA \rightarrow \mathbb{R}$ denotes the reward function, which assigns a scalar score (reward) to an action taken by the agent at a given state; and $S_\mathrm{T}$ denotes the terminal states that stop the process \cite{kaelbling1996reinforcement}.

The objective of RL is to maximize a cumulative reward by finding the agent's optimal policy \cite{article111, inproceedings2222, 10.1145/3152434.3152441}. It seeks to find a balance between acquiring new knowledge (exploration) and using existing knowledge (exploitation) about the environment and the optimal behavior of the agent. A policy is a map $\pi : S\rightarrow A$ that chooses an action $a \in A$ for any given state. A policy may be stochastic, in which case $\pi$ is interpreted as a conditional distribution $\pi(a|s)$ from which actions are sampled.

Each policy induces a state-action function, also known as the Q-function: $Q_\pi(s,a) = \E_\pi [ G_t| S_t=s,A_t = a]=R_s^{a}+\gamma\sum_{s' \in S}P_{ss'}^{a}v_\pi(s'),$
% \begin{equation}
% \begin{gathered}
% Q_\pi(s,a) = \E_\pi [ G_t| S_t=s,A_t = a]=R_s^{a}+\gamma\sum_{s' \in S}P_{ss'}^{a}v_\pi(s'),
% \nonumber
% \end{gathered}
% \end{equation}
%$Q_\pi(s,a) = \E_\pi [ G_t| S_t=s,A_t = a]=R_s^{a}+\gamma\sum_{s' \in S}P_{ss'}^{a}v_\pi(s'),$
where  $R_s^{a}$ is the instant reward that can be obtained by taking
action \(a\) under state \(s\); \(P_{ss'}^{a}\) is the transition probability from state \(s\) to state $s'$ under action \(a\); \(\gamma\) is the discount factor used to balance the long-term and short-term rewards; and \(G_t\) is the cumulative reward from time \(t\), given by $G_t= \sum_{k=0}^{\infty} \gamma^{k} R_{t+k+1}.$
$v_\pi(s) = \E_{\pi} [G_t| s_t=s] = \sum_{a \in A} \pi(a|s)Q_{\pi}(s|a)$. This function is essential for determining the optimal policy. In the case of small state-action spaces, the Q-function can be simply computed and tabulated. However, such an approach quickly becomes infeasible as the cardinality of $S$ and $A$ grows. Deep neural networks were shown to be extremely successful in approximating the values of $Q$ with a reasonable number of trainable parameters.

Broadly speaking, there are two approaches to RL problems: model-based and model-free \cite{9634122}. Model-based learning models the environment and then chooses the optimal policy based on the learned model. In contrast, in model-free learning, the agent establishes the optimal policy through trial and error \cite{9634122}, and the methods are classified into two broad categories: policy optimization techniques and Q-learning value iteration techniques. Q-learning is a model-free RL algorithm that learns the optimal Markov Decision Process policy using Q-values, which estimate the ``value" of taking an action at a given state. In policy optimization, the agent directly learns the policy function that maps state to action, without the use of the value function. Among the algorithms that make use of this method is Trust Region Policy Optimization (TRPO) \cite{schulman2017trust}. TRPO is an on-policy method, which means that it attempts to evaluate or improve the policy that is currently being used to take actions, and it uses information gathered from consecutive steps. It is applicable to both discrete and continuous action spaces, and updates policies by taking the most significant possible step to improve performance while maintaining a degree of similarity between the new and old policies. The latter constraint ensures that the new updated policy remains within the trust region of the old policy:
\begin{equation}
\begin{gathered}
\begin{multlined}
    \max_{\pi'} \E_{\pi'} \left[ \frac{\pi'(a|s)}{\pi(a|s)} \hat{A}_{\pi}(s,a) \right], \\ \mathrm{s.t.} \,\,  \E_{\pi}[D_\mathrm{KL}(\pi(\cdot|s) \, | \, \pi' (\cdot|s))]\leq\delta,
\end{multlined}
\end{gathered}
\label{KL}
\end{equation}where $\pi'$ and $\pi$ denote the new and previous policies, respectively.
$\hat{A}_{\pi}(s,a) \approx Q_{\pi}(s,a) - v_\pi(s)$ 
% \begin{equation}
% \begin{gathered}
% \hat{A}_{\pi}(s,a) \approx Q_{\pi}(s,a) - v_\pi(s) 
% \nonumber
% \end{gathered}
% \end{equation} 
is the approximate advantage function (i.e., the gain in reward relative to the state value when taking a specific action $a$), $D_\mathrm{KL}$ denotes the Kullback-Leibler (KL) divergence between two distributions, and $\delta$ is a fixed radius. The policy and the advantage functions are practically implemented in DRL settings as neural networks parameterized by some parameter vector $\theta$. Equation \ref{KL} can be interpreted as maximizing the objective function that meets the KL constraint term on the policy update step size. The probability ratio between the new policy $\pi_{\theta'}$ and the old one $\pi_{\theta}$ is defined as $r({\theta}') = \frac{\pi_{\theta'}(a|s)}{\pi_{\theta}(a|s)}.$
% \begin{equation}
% r({\theta}') = \frac{\pi_{\theta'}(a|s)}{\pi_{\theta}(a|s)}.
% \nonumber
% \end{equation}
The objective function maximized by TRPO can be defined as $J_{\textrm{TRPO}}(\theta') = \E \left[ r({\theta'}) A_{\theta'}(s,a)\right].
$
% \begin{equation}
% \begin{gathered}
% J_{\textrm{TRPO}}(\theta') = \E \left[ r({\theta'}) A_{\theta'}(s,a)\right].
% \nonumber
% \end{gathered}
% \end{equation}
% \begin{equation}
% \begin{gathered}
% J_{\textrm{TRPO}}(\theta') = \E \left[ r({\theta'}) A_{\theta'}(s,a)\right].
% \nonumber
% \end{gathered}
% \end{equation}

Similarly to TRPO, Proximal Policy Optimization (PPO) \cite{schulman2017proximal} is another on-policy algorithm that seeks to improve the policy without risking performance collapse. Moreover, by limiting policy updates at each training step, PPO improves the stability of the agent's training. PPO is a first-order optimization. In the absence of constraints, the large and small step size updates of the objective function can cause instability or slow convergence. To stay within a small interval around $1$, PPO replaces the complex KL constraint from Eq. \ref{KL} with a projection clipping the policy ratio $r$ \cite{schulman2017proximal},
\begin{equation}
\begin{multlined}
\begin{gathered}
J_\textrm{PPO}(\theta') = \E\left[ \min\{ r({\theta}'), 1+\epsilon\} \hat{A}_{\theta}(s,a)\right].
\nonumber
\end{gathered}
\end{multlined}
\end{equation}
The clipping at $1+\epsilon$ ensures that $J_\textrm{PPO}$ lower bounds $J_{\textrm{TRPO}}$.

==> files/tabeles.tex <==
In this appendix, we present the training statistics of the various AARL agents. Considers first Table \ref{tab:10-links-table}, which shows the statistic for the 10-link topology. We can see that the time it takes for the various AARL agents to converge is approximately 7 hours of training time. For this topology, the batch size is 256 action/state/reward triples. The number of steps required for AARL to converge ranges between 1-2 million steps. The size of the hidden layers of the neural network is 256 neurons for each layer.

Table \ref{tab:48 liinks} presents the same statistics for the 48-link topology. We can see that the time it takes for the various AARL agents to converge is approximately 10 times longer than for the 10-link topology. Although the batch size for this topology was also 256 action/state/reward triples, the number of steps required for AARL to converge is much bigger: between 5.5-7 million steps. Each hidden layer of the neural network contains 1024 neurons.

In Table \ref{tab:96 liinks}, for the 96-link topology, we see similar patterns with respect to training time and size of hidden layers. This time, the number of steps required to reach convergence was not significantly larger than for the 48-link topology, most likely due to a larger batch size that was used.

\begin{table}[H]
\centering
\scalebox{0.93}{
\begin{tabular}{lllll}\toprule
           Agent & \makecell{Steps \\{[}M{]}} & \makecell{Batch \\Size} & NN            & \makecell{Time\\ {[}H{]}} \\
            \midrule 
20-AARL-DI  & 1.1           & 256        & {[}256,256{]} & 4            \\
20-AARL-DS  & 1.2           & 256        & {[}256,256{]} & 4            \\
40-AARL-DI  & 1.3           & 256        & {[}256,256{]} & 3            \\
40-AARL-DS  & 1.4           & 256        & {[}256,256{]} & 7            \\
60-AARL-DI  & 0.8           & 256        & {[}256,256{]} & 9            \\
60-AARL-DS  & 1.6           & 256        & {[}256,256{]} & 12           \\
80-AARL-DI  & 1.9           & 256        & {[}256,256{]} & 7            \\
80-AARL-DS  & 1.8           & 256        & {[}256,256{]} & 13           \\
100-AARL-DI & 2             & 256        & {[}256,256{]} & 8            \\
100-AARL-DS & 2.2           & 256        & {[}256,256{]} & 7         \\
\bottomrule
\end{tabular}}
\caption{Training statistics for the 10-link topology on a uniform workload of packets distribution.}
\label{tab:10-links-table}
\end{table}

\begin{table}[H]
\centering
\scalebox{0.93}{
\begin{tabular}{lllll}\toprule
       Agent     & \makecell{Steps \\{[}M{]}} & \makecell{Batch \\Size} & NN              & \makecell{Time\\ {[}H{]}} \\
            \midrule 
20-AARL-DI  & 7             & 256        & {[}1024,1024{]} & 45           \\
20-AARL-DS  & 6.15          & 256        & {[}1024,1024{]} & 43           \\
40-AARL-DI  & 7             & 256        & {[}1024,1024{]} & 27           \\
40-AARL-DS  & 5.85          & 256        & {[}1024,1024{]} & 38           \\
60-AARL-DI  & 5             & 256        & {[}1024,1024{]} & 39           \\
60-AARL-DS  & 7.25          & 256        & {[}1024,1024{]} & 44           \\
80-AARL-DI  & 5.85          & 256        & {[}1024,1024{]} & 41           \\
80-AARL-DS  & 6.5           & 256        & {[}1024,1024{]} & 44           \\
100-AARL-DI & 6.15          & 256        & {[}1024,1024{]} & 36           \\
100-AARL-DS & 9.2           & 256        & {[}1024,1024{]} & 74          \\
\bottomrule
\end{tabular}}
\caption{Training statistics for the 48-link topology on a uniform workload of packets distribution.}
\label{tab:48 liinks}
\end{table}


\begin{table}[H]

\centering
\scalebox{0.93}{
\begin{tabular}{lllll}\toprule
     Agent       & \makecell{Steps \\{[}M{]}} & \makecell{Batch \\Size} & NN              & \makecell{Time\\ {[}H{]}} \\
            \midrule
20-AARL-DI  & 4             & 512        & {[}4096,4096{]} & 69           \\
20-AARL-DS  & 4.2           & 512        & {[}4096,4096{]} & 72           \\
40-AARL-DI  & 4.5           & 512        & {[}4096,4096{]} & 78           \\
40-AARL-DS  & 4.7           & 512        & {[}4096,4096{]} & 80           \\
60-AARL-DI  & 4.15          & 512        & {[}4096,4096{]} & 84           \\
60-AARL-DS  & 4.8           & 512        & {[}4096,4096{]} & 88           \\
80-AARL-DI  & 4.8           & 512        & {[}4096,4096{]} & 85           \\
80-AARL-DS  & 4.2           & 512        & {[}4096,4096{]} & 80           \\
100-AARL-DI & 5             & 512        & {[}4096,4096{]} & 90           \\
100-AARL-DS & 4.85          & 512        & {[}4096,4096{]} & 92         \\
\bottomrule
\end{tabular}}
\caption{Training statistics for the 96-link topology on a uniform workload of packets distribution.}
\label{tab:96 liinks}
\end{table}


